Optilization of the gyroaverage operator based on hermite interpolation

Gyrokinetic modeling is appropriate for describing Tokamak plasma turbulence, and the gyroaverage operator is a cornerstone of this approach. In a gyrokinetic code, the gyroaveraging scheme needs to be accurate enough to avoid spoiling the data but also requires a low computation cost because it is applied often on the main unknown, the 5D guiding-center distribution function, and on the 3D electric potentials. In the present paper, we improve a gyroaverage scheme based on Hermite interpolation used in the Gysela code. This initial implementation represents a too large fraction of the total execution time. The gyroaverage operator has been reformulated and is now expressed as a matrix-vector product and a cache-friendly algorithm has been setup. Different techniques have been investigated to quicken the computations by more than a factor two. Description of the algorithms is given, together with an analysis of the achieved performance.

==> biblio.tex <==
\bibitem{as} M. \textsc{Abramowitz}, I. A. \textsc{Stegun},
\emph{Handbook of Mathematical Functions},
(Dover Publications, New York, 1965).

\bibitem{bostan2} M. \textsc{Bostan},
\emph{Transport equations with disparate advection fields. Application to the gyrokinetic models in plasmas physics},
J. Differential Equations \textbf{249} (2010) pp. 1620Ð1663.

\bibitem{brizard}
A. \textsc{Brizard},
\emph{Nonlinear gyrokinetic Maxwell-Vlasov equations using magnetic coordinates}
J. Plasma Phys. \textbf{41} (1989), pp. 541Ð559.

\bibitem{besse} D. \textsc{Coulette}, N. \textsc{Besse}
\emph{Numerical comparisons of gyrokinetic multi-water-bag models}.
JCP \textbf{248} (2013), pp. 1Ð32.

\bibitem{cms} N. \textsc{Crouseilles}, M. \textsc{Mehrenberger}, H. \textsc{Sellama},
\emph{Numerical solution of the gyroaverage operator for the finite gyroradius guiding-center model},
CiCP \textbf{8} (2010), pp. 484Ð510.

\bibitem{Dimits_PoP2000} A. \textsc{Dimits} et al.,
\emph{Comparisons and physics basis of tokamak transport models and turbulence simulations},
Physics of Plasmas \textbf{7}, No. 3 (2000), pp. 969Ð983.

\bibitem{Garbet_NF2010} X. \textsc{Garbet}, Y. \textsc{Idomura}, L. \textsc{Villard}, T.H. \textsc{Watanabe},
\emph{Gyrokinetic simulations of turbulent transport},
Nuclear Fusion \textbf{50}, No. 4 (2010), 043002.

\bibitem{gysela2}
V.  \textsc{Grandgirard,} Y. \textsc{Sarazin}, X. \textsc{Garbet}, G. \textsc{Dif-Pradalier}, Ph. \textsc{Ghendrih}, N. \textsc{Crouseilles}, G. \textsc{Latu}, E. 
\textsc{Sonnendr\"ucker}, N. \textsc{Besse}, P. \textsc{Bertrand}, 
\emph{Computing ITG turbulence with a full-f semi-Lagrangian code,} 
Communications in Nonlinear Science and Numerical Simulation \textbf{13} No. 1 (2008), pp. 81Ð87.

\bibitem{gorler} T. \textsc{G\"orler},
\emph{Multiscale effects in plasma microturbulence}, Thse, Ulm (2009).

\bibitem{gene} T. \textsc{G\"orler,} X. \textsc{Lapillonne}, S. \textsc{Brunner}, T. \textsc{Dannert}, F. \textsc{Jenko}, F. \textsc{Merz}, D. \textsc{Told},
\emph{The global version of the gyrokinetic turbulence code GENE.},
J. Comput. Physics \textbf{230}, No. 18 (2011), pp. 7053Ð7071.

\bibitem{Hatzky_PoP2002} R. \textsc{Hatzky}, T.M. \textsc{Tran}, A. \textsc{Konies}, R. \textsc{Kleiber}, S.J. \textsc{Allfrey}, 
\emph{Energy conservation in a nonlinear gyrokinetic particle-in-cell code for ion-temperature-gradient-driven modes in theta-pinch geometry},
Physics of Plasmas \textbf{9}, No. 3 (2002), pp. 898Ð912.

\bibitem{Idomura_NF2003} Y. \textsc{Idomura}, S. \textsc{Tokuda}, Y. \textsc{Kishimoto}, M. \textsc{Wakatani},
\emph{Gyrokinetic theory of drift waves in negative shear tokamaks},
Nuclear Fusion \textbf{41}, No. 4 (2001).

\bibitem{Jolliet_CPC2007} S. \textsc{Jolliet}, A. \textsc{Bottino}, P. \textsc{Angelino}, R. \textsc{Hatzky}, T.M. \textsc{Tran}, B.F. \textsc{Mcmillan}, O. \textsc{Sauter}, K. \textsc{Appert}, Y. \textsc{Idomura}, L. \textsc{Villard},
\emph{A global collisionless PIC code in magnetic coordinates},
Comp. Phys. Comm. \textbf{177}, No. 5 (2007), pp. 409Ð425.

\bibitem{Lee_PFL1983} W. W. \textsc{Lee},
\emph{Gyrokinetic approach in particle simulation},
Physics of Fluids \textbf{26}, No. 2 (1983), pp. 556Ð562.

\bibitem{Li2005} J. \textsc{Li},
\emph{General explicit difference formulas for numerical differentiation},
Journal of Computational and Applied Mathematics \textbf{183} (2005), pp. 29Ð52.

\bibitem{Sarazin_PPCF2005} Y. \textsc{Sarazin}, V. \textsc{Grandgirard}, E. \textsc{Fleurence}, X. \textsc{Garbet}, Ph.  \textsc{Ghendrih}, P. \textsc{Bertrand}, G. \textsc{Depret},
\emph{Kinetic features of interchange turbulence},
Plasma Phys. Control. Fusion \textbf{47}, No. 10 (2005), pp. 1817Ð1840.


\bibitem{Steiner2014} C. \textsc{Steiner}, M. \textsc{Mehrenberger}, N. \textsc{Crouseilles}, V. \textsc{Grandgirard}, G. \textsc{Latu}, F. \textsc{Rozar},
\emph{Gyroaverage operator for a polar mesh},
European Physical Journal D \textbf{69}, No 1, 2015, http://dx.doi.org/10.1140/epjd/e2014-50211-7

\bibitem{bessel}
M. \textsc{Kreh}, 
\emph{Bessel Functions}, www.math.psu.edu/papikian/Kreh.pdf


==> non_regression_test.tex <==


\todo{Explain the test which ensures the correctness of the different versions
of the gyroaverage during the developpement.}

In~\ref{Steiner2014}, different analytical solutions of the
gyroaverage were identified.


